Architectures and circuits for distributed quantum computing

This thesis treats networks providing quantum computation based on distributed paradigms. Compared to architectures relying on one processor, a network promises to be more scalable and less fault-prone. Developing a distributed system able to provide practical quantum computation comes with many challenges, each of which need to be faced with careful analysis in order to create a massive integration of several components properly engineered. In accordance with hardware technologies, currently under construction around the globe, telegates represent the fundamental inter-processor operations. Each telegate consists of several tasks: i) entanglement generation and distribution, ii) local operations, and iii) classical communications. Entanglement generation and distribution is an expensive resource, as it is time-consuming. The main contribution of this thesis is on the definition of compilers that minimize the impact of telegates on the overall fidelity. Specifically, we give rigorous formulations of the subject problem, allowing us to identify the inter-dependence between computation and communication. With the support of some of the best tools for reasoning -- i.e. network optimization, circuit manipulation, group theory and ZX-calculus -- we found new perspectives on the way a distributed quantum computing system should evolve.

==> OLDintroduction/intro.tex <==
\chapter{Introduction (\texttt{due:1/12/2022})}
    \section{Technologies overview}
    \section{Distributed architectures}
            \subsubsection{Multi-core based}
            NISQ architectures are widespread and they promise to be resources of practical interest in the next future. Furthermore, their design is likely to rapidly evolve
            \subsubsection{Farm based}
            \subsubsection{Web based (\texttt{quantum internet})}
    \section{Formalism essentials}
        \subsection{Notation}
            \begin{itemize}
                \item Hilbert space $\mathbb{H}$
                \item Dirac's notation
                \item Density operators
                \item Trace
                \item Oracle complexity
            \end{itemize}
        \subsection{A leap to non-determinism}
            \begin{center}
                \begin{quantikz}[thin lines, row sep={0.7cm,between origins}, column sep={0.4cm}]
                    \lstick{$_{{b}}$}& \qw& \gate[style={fill=lime!10}]{_{\lnot}} & \qw& \qw \rstick[]{$_{\lnot {b}}$}
                \end{quantikz}
            \end{center}
            \begin{center}
                \begin{quantikz}[thin lines, row sep={0.7cm,between origins}, column sep={0.4cm}]
                    \lstick{$_{\ket{\varphi}}$}& \qw& \gate[style={fill=lime!10}]{_{\texttt{X}}} & \qw& \qw \rstick[]{$_{\texttt{X}\ket{\varphi}}$}
                \end{quantikz}
            \end{center}
            A state $\ket{\varphi}$ can be equivalently expressed as $\ket{\varphi}\bra{\varphi}$, said to be \textbf{pure}. 
            Now that it lays on a wider space, we can represent also states affected by noise.
            Let us introduce the \textit{density} state:
            \[\sigma = \sum_k \texttt{p}_k\ket{\varphi_k}\bra{\varphi_k}.\]
            Any state affected by noise can be expressed as a mixture of pure states.
            \begin{center}
                \begin{quantikz}[thin lines, row sep={0.7cm,between origins}, column sep={0.4cm}]
                    \lstick{$_{b}$}& \qw& \gate[style={fill=lime!10}]{_{\{\lnot, \mathds{1}\}}} & \qw& \qw \rstick[]{$_{\texttt{p} \cdot\lnot b + (1-\texttt{p})\cdot b}$}
                \end{quantikz}
            \end{center}
            \begin{center}
                \begin{quantikz}[thin lines, row sep={0.7cm,between origins}, column sep={0.4cm}]
                    \lstick{$_{\sigma}$}& \qw& \gate[style={fill=lime!10}]{_{\{\texttt{X}, \mathds{1}\}}} & \qw& \qw \rstick[]{$_{\texttt{p} \cdot \texttt{X}\sigma\texttt{X} + (1-\texttt{p})\cdot\sigma}$}
                \end{quantikz}
            \end{center}
            where $\texttt{X} \equiv \ket{\texttt{0}}\bra{\texttt{1}} + \ket{\texttt{1}}\bra{\texttt{0}}$.
            
    \section{Main challenges}
        %NISQ-era
        \subsection{Universal computing}
        \subsection{Resource optimization}
            \subsubsection{Compiling (\texttt{ACM Trans.})}



        

==> compilation/old.tex <==
\subsection{Adapting the model to literature}
\subsubsection{Time-expansion}
\label{sec:time-exp}
Formulation \eqref{dqcc} is a particular case of \texttt{MCF}$_d$, as it slightly recedes from the standard formulation.
As expected, the problem is still intractable. To understand that, consider this simple scenario: an instance $[k]$ with $k=2$ such that $1\shortparallel2$. We can restate the problem as follows: assert if there exists a solution at first time step. If not, just put operation $2$ at second time step. Unfortunately, asserting if such a solution exists is \texttt{NP}-hard. Indeed, in Ref. \cite{EveItaSha-75}, authors proved the hardness of such a decision problem, even for single capacity edges. Therefore, it is reasonable to look for approximations of \texttt{DQCC}. To this aim, we think a good line of research would be to follow a common technique for tackling $\texttt{MCF}_d$: the \textit{time-expansion} \cite{ForFul-58}. Please refer to \cite{cuomo2021optimized} for a detailed implementation proposal.

==> introduction/intro.tex <==
\chapter{Introduction}
\label{ch:techs}
\thispagestyle{empty}
\newpage

Distributed quantum computing is one of the most appealing applications in the panorama of quantum technologies. In fact, distributed architectures could be our bridge to step beyond the current NISQ era \cite{Preskill2018, cuomo2020towards, gibney2019quantum, gambetta2020ibm, CacCalTaf-19,VanDev-16}. This explains the wide interest for a large-scale integration of quantum technologies. By inter-connecting spatially distributed quantum processors, we would achieve a scalable architecture resistant to noise. The general trend \cite{gambetta2020ibm, eddins2022doubling, liu2022design, gold2021entanglement, kielpinski2002architecture, stephenson2020high} shows a common belief in distributed \textcolor{black}{(and quasi-distributed, or multi-core)} architectures as physical substrate, allowing a modular and horizontal scale-up of computing resources, rather than relying on vertical scale-up, coming from single hardware advancements.
%On contrary, linking several quantum processors, spatially distributed, makes the scale up achievable, i.e., a horizontal scale up. EP: SAREBBE MOLTO CONTESTABILE AFFERMARE CHE NESSUNA TECNOLOGIA HARDWARE SIA  DI PER SE' SCALABILE.  
%As usual in distributed architectures, several processors are located in spatially remote places and they need to exchange information to work together.
On the flip side, by linking distributed quantum processors, several new challenges arise \cite{Kim-08,PirBra-16,DurLamHeu-17,WehElkHan-18,Cas-18,cuomo2020towards}.

Being up-to-date with technologies currently under construction around the globe is a mandatory step to create a realistic system. We hence begin -- in Sec. \ref{sec:tech} -- by reviewing some of the most promising hardware technologies. This provide us (and the reader) with a realistic perspective of the fundamental components belonging a distributed quantum computing system. Once done that we propose -- in Sec. \ref{sec:stack} -- a full-stack development meant to be modular and prone to future changes. %, as it naturally happens in fields where new discoveries are ordinary.
 The stack is indeed already an extension of one of our first proposal, available in \cite{cuomo2020towards}.

In Ch. \ref{ch:essentials}, we abstract from hardware technologies, by introducing the reader to the fundamental tools concerning distributed computing paradigms. We use the most affirmed language to express quantum computation, i.e. the standard quantum circuit model. We start with some basics on unitary \textit{synthesis} and \textit{decomposition}, important also for local computational. We then extend the subject to work on distributed architectures.

For the sake of completeness, In Ch. \ref{ch:noise} we provide a framework concerning quantum noise. Handling noise is probably, to date, the hardest challenge we are facing, as any model struggle to be scalable for hardware. Hence the aim of this chapter is to give a perspective of the magnitude of the problem, which -- sooner or later -- will be part of a distributed computing system. The framework is strengthen by experimental results.

We conclude the thesis with what is our main contribution to research. Thanks to the knowledge gathered by us throughout the aforementioned chapters, we could minutely investigate one essential component for any system implementation of practical value. Such a component is commonly referred as \textit{compiler}, which we formulate with mathematical rigor in Ch. \ref{ch:compile}.
With the support of some of the best tools for reasoning -- i.e. network optimization, circuit manipulation, group theory and \texttt{ZX}-calculus -- we managed to give a first complete model for the compilation problem on distributed architectures. Every feature characterizing the problem is treated minutely. We could separate the problem in several parts, each of which is tackled with a dedicated optimizer.

We also use our model as benchmarker for different network topologies. It is indeed important, in the development of a practical system, that the project follows a \textit{co-design} line, where each component is designed to fit at its best with the other components.

==> logic/old.tex <==

\section{Entanglement-assisted stabilizer groups}
Coming back to the importance of classical codes. So far we restricted the focus on particular sub-groups of classical linear codes. The reason, as already explained in Sec. \ref{sec:classic-codes}, is an interest to find a generic way for mapping classical codes to stabilizer codes. In this sense we pointed out how any linear code which is self-orthogonal has a correspondent stabilizer code. 

Consider a generic linear codes $\Sigma_{k,m}$. we reviewed how to construct a stabilizer code $\Gamma_{k-m,m}$ by means of $H_{\Sigma}$. Assume $\Sigma$ to not satisfying self-orthogonality. Then $H_{\Gamma}$ relate to one or more pairs of non-commuting stabilizer, i.e. $H_{\Gamma}^{\ }H_{\Gamma}^{\intercal} \neq 0$.

The \textit{entanglement-assisted stabilizer} theory \cite{djordjevic2021quantum} allows to use $\Sigma_{k,m}$ and getting a new code $\bar{\Gamma}_{k-m, m-c, c}$, passing by $\Gamma_{k-m,m}$. The framework introduces $c$ auxiliary qubits to the code, which are also assumed to be maximally entangled to as many of the $m$ original auxiliary qubits -- explaining the change from $m$ to $m-c$. The choice of $c$ is optimal and can be easily verified as it corresponds to the rank of $H_{\Gamma}^{\ }H_{\Gamma}^{\intercal}$ \cite{hsieh2007general, calderbank1998quantum}.

The importance of using entanglement pairs comes from the fact that we can simplify the noise model acting on maximally entangled states, as these have a very appealing property. 

\subsubsection{Noise over entangled states}
Consider a generic Bell pair $\ket{\Phi^{\texttt{+}}}_{ij}$; the noise affecting its system can be described by a set of operators in \[\mathbb{E}_{i} \equiv \{\texttt{I}_i, \texttt{X}_i, \texttt{Z}_i, \texttt{X}_i\texttt{Z}_i\},\]
which can be read as operators affecting only half of the system. To see that, notice that operators $\texttt{I}_{ij}$, $\texttt{X}_{ij}$, $\texttt{Z}_{ij}$ and $\texttt{X}_{ij}\texttt{Z}_{ij}$ do not affect $\ket{\Phi^{\texttt{+}}}_{ij}$.
As regard less trivial operators, take $\texttt{Z}_i\texttt{X}_{j}\texttt{Z}_{j}$ as an example. First notice that $\texttt{Z}_i\texttt{X}_{j}\texttt{Z}_{j} \equiv \texttt{Z}_{ij}\texttt{X}_{j}$ and $\texttt{Z}_{ij}$ has no role. Furthermore, $\texttt{X}_j\ket{\Phi^{\texttt{+}}}_{ij} \equiv \texttt{X}_i\ket{\Phi^{\texttt{+}}}_{ij} \equiv \ket{\Psi^{\texttt{+}}}_{ij}$, as desired. This is also true for the remaining operators, being aware that $\texttt{Z}_j\ket{\Phi^{\texttt{+}}}_{ij} \equiv \texttt{Z}_i\ket{\Phi^{\texttt{+}}}_{ij} \equiv \ket{\Phi^{\texttt{-}}}_{ij}$. %As consequence, a generic error operator $\texttt{E}$, acting on $\texttt{Im}(\Gamma_{k,m,\ell})$ is such that

The subject framework -- outlined in next subsection -- works under the (non-restrictive) assumption that a generic noise issues operators $\texttt{E} \in \mathbb{E}\otimes\mathbb{E}_i$.

\subsubsection{Generation method}
The \textit{symplectic Gram-Schmidt orthogonalization algorithm} \cite{shaw2010quantum} takes in input $H_{\Gamma}$ and outputs two matrices $\bar{H}$ and $\bar{\bar{H}}$ which are isomorphic under some Clifford transformation. $\bar{\bar{H}}$ relates to a canonical set of stabilizer generators, as they correspond to single qubit operators of $\mathbb{E}$. For this reason, it is used to easily spot where a couple of stabilizers anti-commute and, based on that, one can build a matrix $A$ composed by $c$ columns. Each column of $A$ is meant to turn a couple of anti-commuting rows of $\bar{\bar{H}}$ into a commuting one.
Since $\bar{H}$ and $\bar{\bar{H}}$ are isomorphic, $A$ can be used to get the final matrix
\begin{equation}
    H_{\bar{\Gamma}} = (A|\bar{H})
\end{equation}
By construction, $H_{\bar{\Gamma}}$ inherits the error-correcting properties of $H_{\Gamma}$. Furthermore, $H_{\bar{\Gamma}}$ relates to an abelian stabilizer group still composed by operators in $\mathbb{E}$. Hence, the transversal implementations of
$\pmb{\land(\texttt{{X}})}, \pmb{\texttt{X}^{\sfrac{1}{2}}}$ or $\pmb{\texttt{Z}^{\sfrac{1}{2}}}$ are logical operators for $\bar{\Gamma}$.

The result is a framework enabling \textit{entanglement-assisted fault-tolerant computing}, by means of any linear code.
The previously needed self-orthogonality of linear codes is a substantial obstacle to import the linear coding theory in its entirety, especially in the context of most efficient codes such as low-density parity-check codes \cite{berrou1993near} and turbo codes \cite{gallager1962low}. Having access to any linear code is generally good, as the better the classical code is, the better its “quantization” will be \cite{brun2006correcting}.

==> preface.tex <==
\chapter*{\centering {\large Preface}}
\begin{figure}[h]
        \centering
        \begin{minipage}[c]{.23\textwidth}
        \centering
            \includegraphics[scale=0.047]{ibm_logo.png}
        \end{minipage}
        \begin{minipage}[c]{.23\textwidth}
        \centering
            \includegraphics[scale=0.089]{cnr_logo.png}
        \end{minipage}
        \begin{minipage}[c]{.23\textwidth}
        \centering
            \includegraphics[scale=0.072]{polimi_logo.png}
        \end{minipage}
        \begin{minipage}[c]{.23\textwidth}
        \centering
            \includegraphics[scale=0.015]{uc3m_logo.png}
        \end{minipage}\\[0.7cm]
        \begin{minipage}[c]{.23\textwidth}
        \centering
            \includegraphics[scale=0.034]{unicam_logo.png}
        \end{minipage}
        \begin{minipage}[c]{.23\textwidth}
        \centering
            \includegraphics[scale=0.057]{unina_logo.png}
        \end{minipage}
        \begin{minipage}[c]{.23\textwidth}
        \centering
            \includegraphics[scale=0.054]{NuQ_logo.png}
        \end{minipage}
        \begin{minipage}[c]{.23\textwidth}
        \centering
            \includegraphics[scale=0.025]{unimi_logo.png}
        \end{minipage}
\end{figure}

==> quote.tex <==
\newpage

\null\vfill
%\epigraph{Listen to the scientists.}{\textit{Greta Thunberg}}
%\epigraph{To those creatures that are fading away.\\ I am coming for you.}{}
\epigraph{\textit{Endless forms,}\\ \textit{unified tapestry of creation.}}{}
\thispagestyle{empty}
\newpage

==> resources/OLD.tex <==
\begin{exmp}
    Consider the $\texttt{ZZ}(\alpha)$ Ising gate:
    \begin{center}
        \begin{quantikz}[thin lines, row sep={0.7cm,between origins}, column sep={0.4cm}]
            &\gate[2,style={fill=violet!10}]{_{\texttt{ZZ}(\alpha)}}&\qw\\
            &&\qw
        \end{quantikz}
    \end{center}
    Since $\alpha = \beta$ and $\delta = 0$, the corresponding gate synthesis is:
    \begin{center}
        \begin{quantikz}[thin lines, row sep={0.3cm,between origins}, column sep={0.4cm}]
            & \ctrl{2} & \qw & \ctrl{2} & \qw &\qw& & & \ctrl{2} & \gate[style={fill=cyan!10}]{_{\texttt{Z}_{\alpha}}} & \ctrl{2} & \qw\\
            & & & & & &\ \equiv\ & & & & & &\\
            & \targ{} & \gate[style={fill=cyan!10}]{_{\texttt{Z}_{\texttt{-}\alpha}}} & \targ{} & \gate[style={fill=cyan!10}]{_{\texttt{Z}_{\alpha}}} &\qw & & & \targ{} &\qw & \targ{} &\qw
        \end{quantikz}
            
    \end{center}
\end{exmp}
            
            
\begin{equation*}
    \frac{1}{4}
        \arraycolsep=1.5pt\begin{bmatrix} 
                _{|\alpha|^2 + |\beta|^2} & _{|\alpha|^2} & _{0} & _{\beta\alpha^*} \\
                _{|\alpha|^2} & _{|\alpha|^2 + |\beta|^2} &    _{\beta\alpha^*} & _{0}\\
                _{0} & _{\alpha\beta^*} & _{|\alpha|^2 + |\beta|^2} & _{|\beta|^2}\\
                _{\alpha\beta^*} & _{0} & _{|\beta|^2} & _{|\alpha|^2 + |\beta|^2}
            \end{bmatrix}.
\end{equation*}


      \subsection{State injection}
            \begin{figure}[h]
                \centering
                \begin{quantikz}[thin lines]
                    \lstick[]{$_{\ket{\varphi}}$}&\ctrl{1}&\gate[style={fill=cyan!10}]{_{\texttt{Z}_{\sfrac{\pi}{2}}}}&\qw \rstick[]{$_{\texttt{Z}_{\sfrac{\pi}{4}}\ket{\varphi}}$}\\
                    \lstick[]{$_{\ket{\omega}}$}&\targ{}&\ctrl{-1}&\qw \rstick[]{$_{\ket{\omega}}$}
                \end{quantikz}
                \caption{Example of $\texttt{Z}_{\sfrac{\pi}{4}}$ \textit{injection}: this holds for any state $\ket{\varphi}$.}
                \label{fig:inj}
                %\hrulefill
            \end{figure}



 A computing paradigm is called measurement-based whenever the quantum computation is interleaved by measurements acting on a sub-system \cite{nielsen2003quantum}. The output of a measurement is then used to perform classical conditioned quantum operations.
        %To describe such a computing paradigm, we were inspired by the formalism used in \cite{djordjevic2021quantum}.
        
        A measurement over a Pauli axis $\bar{\texttt{E}}$ generates a Boolean string $\texttt{o}$:
        \begin{center}
                \begin{quantikz}[row sep={0.7cm,between origins}, column sep={0.4cm}]
                    &\measure[style={fill=lime!10}]{_{\langle \bar{\texttt{E}}\rangle,\texttt{o}}}
                \end{quantikz}
        \end{center}
        The output can then be used to choose whether performing or not a Pauli operation over another qubit:
        \begin{center}
                \begin{quantikz}[row sep={0.7cm,between origins}, column sep={0.4cm}]
                    &\gate[style={fill=lime!10}]{_{\texttt{E}(\texttt{o})}}&\qw
                \end{quantikz}
        \end{center}
        When the boolean string corresponds to a single bit in $\{\texttt{0}, \texttt{1}\}$, then $\texttt{E}$ operates over a single qubit and we have the correspondence $\texttt{E}(\texttt{o}) \equiv \texttt{E}^{\texttt{o}}$. For higher dimensionality $d$, then $\texttt{o} = \texttt{o}_1\texttt{o}_2\cdots\texttt{o}_{\log{d}}$ and $\texttt{E}(\texttt{o}) \equiv \texttt{E}^{\texttt{o}_1}\otimes\texttt{E}^{\texttt{o}_2}\otimes\cdots\otimes\texttt{E}^{\texttt{o}_{\log{d}}}$.

    Entanglement is probably the most fascinating property coming from quantum mechanics. It is also the most promising resource.
    
    To our purpose we focus on one of the four Bell's states. These states are fully entangled, meaning that their correlation is maximal and completely isolated from the environment.
    Let us introduce the $\ket{\Phi^{+}}$ state, defined as follow:
    \[\ket{\Phi^{\texttt{+}}} = \frac{1}{\sqrt{2}}(\ket{\texttt{00}} + \ket{11}).\]
    Since the two system in $\ket{\Phi^{\texttt{+}}}$ present a \textit{non-local} correlation, this state can be used to perform non-local operations. Physically speaking, this means that one need to perform what is called \textit{entanglement generation and distribution} \cite{cacciapuoti2019quantum, cacciapuoti2020entanglement, cuomo2020towards}:
    \begin{itemize}
        \item generation; despite the non-local correlation, the generation happens between system which are in proximity one another. Generating a maximally entangled state with high fidelity is in general hard and time-consuming.
        \item distribution; once the entangled is ready, it is possible to relocate the two systems. The entanglement is, in principle, preserved.
    \end{itemize}
    Below we outline some of the most promising resources for distributed quantum computing, all exploiting entanglement. Most of what follows comes from the work published in \cite{cuomo2021optimized}.




    \begin{wrapfigure}{r}{5cm}
    \centering
    \begin{quantikz}[thin lines, row sep={0.7cm,between origins}, column sep={0.4cm}]
        \lstick[]{$_{\ket{\varphi}}$}& \ctrl{1}\gategroup[wires=2,steps=3,style={draw=none,rounded corners,inner xsep=8pt,inner ysep=-1pt, fill=green!10}, background, label style={rounded corners,label position=above, xshift = 2.5cm,  yshift=-0.85cm, fill=green!10}, background]{$_{P_i}$} &\qw & \gate[style={fill=green!10}]{_{\texttt{Z}^{\texttt{b}_2}}} &  \qw \\
        \lstick[2]{$_{\ket{\Phi^{\texttt{+}}}}$}& \targ{} & \measure[style={fill=green!10}]{_{\langle {\texttt{Z}}\rangle,\ \texttt{b}_1}} \\
        & \ctrl{2}\gategroup[wires=3,steps=3,style={draw=none,rounded corners,inner xsep=8pt,inner ysep=-1pt, fill=red!10}, background, label style=        {rounded corners,label position=above, xshift = 2.5cm,  yshift=-1.2cm, fill=red!10}, background]{$_{P_j}$} & \measure[style={fill=red!10}]{_{\langle {\texttt{X}}\rangle,\ \texttt{b}_2}}\\
        \lstick[]{$_{\ket{\vartheta}}$}  & \targ{} & \qw & \gate[style={fill=red!10}]{_{\texttt{X}^{\texttt{b}_1}}} & \qw\\
        \lstick[]{$_{\ket{\psi}}$}  & \targ{} & \qw & \gate[style={fill=red!10}]{_{\texttt{X}^{\texttt{b}_1}}} & \qw 
    \end{quantikz}
    \caption{Tele-gate performing $\land(\texttt{X}\otimes\texttt{X})$.}
    \label{fig:rcxx}
    \hrulefill
\end{wrapfigure}

==> tec-integration/old.tex <==
\subsection{Qubit-qubit systems: from local to distributed interactions}
\begin{wrapfigure}{r}{6cm}
    \centering
    \input{tec-integration/figures/two-levels.tex}
    \caption{Cyclic two-levels system.}
    \label{fig:2-levels}
    \hrulefill
\end{wrapfigure}
To start understanding how to create a qubit-qubit interaction between distributed systems, it is useful to start from how this usually happens when considering qubits stored within a single processor. %In fact, the two cases have a common denominator: they both relies on some \textit{fermionic mode}. Qualitatively speaking, a qubit is described as a \textit{bosonic mode}, which is a two-level system -- see Fig. \ref{fig:2-levels} --.

In a survey on the state-of-the art of superconducting qubits -- see Ref. \cite{kjaergaard2020superconducting} -- authors identified three main classes of techniques to (locally) entangle qubits. All these techniques drives a \textit{target} qubits depending on the state of a \textit{control} qubit.

One can notice that, among the big array of techniques, some of these rely on a \textit{(virtual) photon mode} which mediates the interaction between the qubits \cite{lauk2020perspectives}.

 \begin{wrapfigure}{r}{6cm}
        \centering
        \input{tec-integration/figures/three-levels.tex}
        \caption{Cyclic three-levels system.}
        \label{fig:3-levels}
        \hrulefill
    \end{wrapfigure}
Depending on the technology mechanics, one can layer a qubit system in a number of ways. Starting from the classification introduced in the survey in Ref. \cite{gu2017microwave}, we identified two main settings useful to understand how to step from local processors to distributed architectures. The two systems are reported in Figs. \ref{fig:2-levels} and \ref{fig:3-levels}.

In the two-level system -- Fig. \ref{fig:2-levels} -- when a qubit is lowered to the ground state, this causes a charge exchange with the mode, which in turns leads the system qubit-mode-qubit to be in a superposition in time of the states $\ket{\texttt{1},n,\texttt{0}}$,$\ket{\texttt{0},n+1,\texttt{0}}$ and $\ket{\texttt{0},n,\texttt{1}}$. Such a configuration lasts for a short time, as the intermediate mode quickly rejects the extra charge, absorbed by the target qubit. Hence, the system can be simplified as a direct coupling of the two qubit, e.g.:
\begin{equation}
    \label{eq:local-interaction}
    \frac{1}{\sqrt{2}}(\ket{\texttt{1},\texttt{0}} + \ket{\texttt{0},\texttt{1}}).
\end{equation}
%This technique leads the foundation of any kind of logical interaction useful to quantum computation. 
This technique does not limit to local processors, but it is also paving the way for \textit{multi-core} architectures \cite{kielpinski2002architecture,fang2014one,ZhoWanZou-20,KraRanHam-21,gold2021entanglement}.
% This can also lead to qubits placed to arbitrary distance, up to be part of the envisioned \textit{quantum internet} \cite{kimble2008quantum}.

Depending on the specific setting, the qubit-qubit interaction may bring to different maximally entangling gates.

To give a practical example, let us consider the \texttt{IBM} superconductor systems, the qubit-qubit coupling occurs by means of a bus mode \cite{rzx-gate}. To see its relation to equation \eqref{eq:local-interaction}, let us start from the state $\ket{\texttt{i},\texttt{i}}$. The two-qubit gate \cite{ibm-resonance} generates the maximally entangled state
\begin{equation}
    -\frac{\texttt{i}}{\sqrt{2}}(\ket{\texttt{1},\texttt{0}} + \ket{\texttt{0},\texttt{1}}),
\end{equation}
which differs from \eqref{eq:local-interaction} by a global phase.

%Now consider the \texttt{IonQ} ion-traps \cite{molmer1999multiparticle,ms-gate}, where the qubits coupling occurs by means of a ``chain's normal modes of motion''. The operator is referred as an \textit{Ising gate}, which superposes two qubits. To see how it relates to our explanation, consider two-qubits prepared in the state $\ket{\texttt{0},\texttt{0}}$. The Ising gate superposes them in the maximally entangled state
%\begin{equation}
%    \frac{1}{\sqrt{2}}(\ket{\texttt{0},\texttt{0}} + \ket{\texttt{1},\texttt{1}}),
%\end{equation}
%which is equivalent to equation \eqref{eq:local-interaction} up to a local bit-flip of one of the two qubits.



==> tikzlibraryquantikz.code.tex <==
%This is the quantikz library for typesetting quantum circuits using LaTeX/Tikz. version 0.9.4
% Written by Alastair Kay, 2018. Published under a CC-BY-4.0 licence
% Please email me (alastair.kay@rhul.ac.uk) with any bug reports or feature requests.
% If you find this library useful, please cite its usage in your work, using arXiv:1809.03842, and possibly the DOI: 10.17637/rh.7000520.
% Usage is at your own risk.

%version 0.9.5:
%	fixed bug which meant multi-wire gates didn't work outside of an environment such as center.
%version 0.9.4:
%	added nwires and cwires options to gate command to simulate qcircuit's nphantom and cphantom
%	vertical text options for slice labels.
%	replaced macro for measuring width and height for greater reliability. disable auto spacing now unnecessary as things like \sqrt{} work in the gate label.
%	investigated possibility of high labels (multi-line labels, particularly for a multi-qubit gate). key disable auto height introduced.
%	now provides a quantikz environment, which is theoretically compatible with tikz' external library (entirely untested). Can still use tikzcd environment otherwise.
%	removed a tikzcd customisation fixing the baseline for one row circuits as this was messing with any manual attempts to adjust the baseline.
%version 0.9.3:
%	adjusted spacing of gate operation between in-circuit and overlay so that transparency looks better
%	Other gate spacing adjustments. multi-qubit gates in particular should look better. 'disable auto spacing' can switch this off, particularly for use with things like \sqrt{} in the multi-qubit gate label, which will throw a weird error.
%	gate command now takes two further optional parameters: minimum width and minimum height for each cell.
%	some consolidation of styling commands
%	global keys 'transparent' and 'thin lines' added. 'thin lines' gives a look more similar to the original QCircuit.
%version 0.9.2:
%	made 'wires' the default key, so [wires=2] now becomes [2]
%	added 'slice title', 'slices style', 'slices label style' key to control titles of slices under 'slice all'
%	better access to positioning of gategroup label.
%	now arXiv compatible (that was a challenge! they use old versions of packages)
%Previous versions:
%version 0.9.1:
%	added \cwbend gate for cornering classical wires.
%	made size of strike through for multiqubit gates stylable via the keys /quantikz/Strike Height/ and /quantikz/Strike Width/
%	added new \gate[swap] variant of swap (nearest-neighbour only).
%version 0.9.0:
%original release.

\ProvidesPackage{quantikz}[2019/04/24 typeset quantum circuit diagrams]

% Package(s) to include
\RequirePackage{xargs,ifthen,xstring,xparse,etoolbox,mathtools}
\RequirePackage{environ} %in an attempt to help with compatibility with the external library of tikz.
\RequirePackage{tikz}
\usetikzlibrary{cd,decorations.pathreplacing,calc,positioning,fit,shapes.symbols,decorations.pathmorphing,shapes.misc,backgrounds,decorations.markings}

\newlength{\myl}
\newlength{\myh}
\newlength{\myd}

%\makeatletter
\newcounter{aaa}
\tikzset{
  apply/.style args={#1 except on segments #2}{postaction={
      /utils/exec={
        \@for\mattempa:=#2\do{\csdef{aaa@\mattempa}{}}
        \setcounter{aaa}{0}
      },
      decorate,decoration={show path construction,
        moveto code={},
        lineto code={
          \stepcounter{aaa}
          \ifcsdef{aaa@\theaaa}{}{
            \path[#1] (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast);
          }
        },
        curveto code={
          \stepcounter{aaa}
          \ifcsdef{aaa@\theaaa}{}{
            \path [#1] (\tikzinputsegmentfirst) .. controls
            (\tikzinputsegmentsupporta) and (\tikzinputsegmentsupportb)
            ..(\tikzinputsegmentlast);
          }
        },
        closepath code={
          \stepcounter{aaa}
          \ifcsdef{aaa@\theaaa}{}{
            \path [#1] (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast);
          }
        },
      },
    },
  },
}
%test if item is in list of item. Probably better ways to do this, but I could get this version to work.
\newcommand*{\IfInList}[2]{%
	\gdef\memory{0}
	\edef\arg{#1}
	 \foreach \q in #2 {%
	 	\ifthenelse{\q=\arg}{%
	 		\gdef\memory{1}
	 	}{}
	 }
	\ifthenelse{\memory=1} {%
		\expandafter\@firstoftwo
	}{%
		\expandafter\@secondoftwo
	}
}
%define the quantikz environment. I need this to facilitate the external library
\NewEnviron{quantikz}[1][]{%
  \def\@temp{\tikzcd@[#1]\BODY}%
  \expandafter\@temp\endtikzcd
}
\def\temp{&} \catcode`&=\active \let&=\temp
%
%commands for putting in text vertically
\protected\def\vvv#1{\leavevmode\bgroup\vbox\bgroup\xvvv#1\relax}
%
\def\xvvv{\afterassignment\xxvvv\let\tmp= }
%
\def\xxvvv{%
% \ifx\tmp\@sptoken\egroup\ \vbox\bgroup\let\next\xvvv
% \else
\ifx\tmp\relax\egroup\egroup\let\next\relax
 \else
\hbox to 1.1em{\hfill\tmp\hfill}% centred
\let\next\xvvv\fi%\fi
\next}
%end of commands for putting text vertically
%
\long\def\ifnodedefined#1#2#3{%
    \@ifundefined{pgf@sh@ns@#1}{#3}{#2}%
}
%I don't think this is used any more
% \newcommand\getwidth[1]{
% 	\pgfkeys{minimum width=0pt}%
% 	\pgfkeys{/quantikz,#1}
% 	\pgfkeysgetvalue{/quantikz/minimum width}{\minwidth}
% 	\minwidth
% }

%the main gate command
\DeclareExpandableDocumentCommand{\gate}{O{}O{1.5pt}O{1.5pt}m}{%optional parameter contains styling info. compulsory is gate text.
	|[inner sep=4pt,minimum width=#2,minimum height=#3]|%
 	\edef\n{\the\pgfmatrixcurrentrow} %the row
 	\edef\m{\the\pgfmatrixcurrentcolumn} %the column
 	%reset macros that are going to be set by the options
 	\edef\options{row=\n,col=\m,#1}
 	\def\toswap{0}%
 	\def\DisableMinSize{0}%
 	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}%
 	%import options passed as parameters
  	\pgfkeys{/quantikz,#1}%
 	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
 	\pgfkeysgetvalue{/quantikz/style}{\a}
 	\pgfkeysgetvalue{/quantikz/label style}{\b}
 	\pgfkeysgetvalue{/quantikz/cwires}{\mylist}
 	\pgfkeysgetvalue{/quantikz/nwires}{\nowires}
 	\ifthenelse{\toswap=1}{%if it's a swap gate...
 		\def\quantwires{2}
 		\phantom{wide}
 		\settowidth{\myl}{$wide$}
 		\settoheight{\myh}{$wide$}
 		\settodepth{\myd}{$wide$}
 	}{%not a swap gate
 		\settowidth{\myl}{$#4$}
 		\ifthenelse{\DisableMinSize=1}{%disable automatic size detection. Use $U$ instead.
 			\phantom{U}
 			\settoheight{\myh}{$U$}
 			\settodepth{\myd}{$U$}
 		}{%automatically get width and height of label
 			\phantom{#4}
 			\settoheight{\myh}{$#4$}
 			\settodepth{\myd}{$#4$}
 		}
 	}
%	
 	\IfInList{1}{\mylist}{\cw}{\IfInList{1}{\nowires}{}{\qw}}%do we need classical, no wire, or quantum wire?
 	\edef\k{\the\numexpr\n+\quantwires-1\relax}
 	\edef\mn{\the\numexpr\m-1\relax}
 	\ifthenelse{\quantwires=1}{}{%more than 1 wire on gate. iterate through each wire
 	\foreach \i in {\the\numexpr\n+1\relax,...,\k} {
 	    \edef\newcom{\noexpand\vcwhexplicit{\i-\m}{\i-\mn}}
       	\edef\newcomb{\noexpand\vqwexplicit{\i-\m}{\i-\mn}}
 	 	\edef\val{\the\numexpr\i+1-\n\relax}
 		\IfInList{\val}{\mylist}{\newcom}{\IfInList{\val}{\nowires}{}{\newcomb}}%do we need classical, no wire, or quantum wire?
 		%apply auto width to the cell, and make sure we unset the setting so that it doesn't apply to later circuits.
 		\globaldefs=1
 		\edef\dotikzset{\noexpand\tikzset{row \i\space column \m/.append style={minimum width={max(\the\myl+8pt,#2)}}}}
 		\dotikzset
 		\edef\undotikzset{\noexpand\tikzset{row \i\space column \m/.style={}}}
      	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendglobals\expandafter{\undotikzset}
 	}
 			%apply auto height to last row only. unsetting already handled above.
 		   \globaldefs=1
 		   \edef\dotikzset{\noexpand\tikzset{row \k\space column \m/.append style={minimum height={max(\the\myh+\the\myd+8pt,#3)}}}}
 		   \dotikzset
%		
 	}
 	%call deferred gate command.
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendsavedpaths\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\gate@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\a\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\b\expandafter}\expandafter{\options}{#4}
	}
}

%deferred gate command. draws a box around all included cells. this is not part of the matrix, but comes afterwards.
\newcommand{\gate@end}[4]{
	\pgfkeys{/quantikz,wires=1}
	\def\toswap{0}
	\def\DisableMinSize{0}
 	\pgfkeys{/quantikz,#3}%
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
	\ifthenelse{\toswap=1}{\def\quantwires{2}}{}
	\xdef\LoopGG{}
	\foreach \n in  {\row,...,\the\numexpr\row+\quantwires-1\relax} {
	\ifnodedefined{\tikzcdmatrixname-\n-\col}{
		\xdef\LoopGG{\LoopGG(\tikzcdmatrixname-\n-\col)}
		}{}
	}
	\ifthenelse{\toswap=1}{
		\node (group\tikzcdmatrixname-\row-\col) [fit=\LoopGG,operator,inner sep=0pt,#1] {\hphantom{Wide}};
		\draw [thickness] (group\tikzcdmatrixname-\row-\col.west|-\tikzcdmatrixname-\row-\col.center) to[out=0,in=180] (group\tikzcdmatrixname-\row-\col.east|-\tikzcdmatrixname-\the\numexpr\row+1\relax-\col.center);
		\draw [line width=3pt,white,shorten >=0.9pt,shorten <=0.9pt] (group\tikzcdmatrixname-\row-\col.east|-\tikzcdmatrixname-\row-\col.center) to[out=180,in=0] (group\tikzcdmatrixname-\row-\col.west|-\tikzcdmatrixname-\the\numexpr\row+1\relax-\col.center);
		\draw [thickness] (group\tikzcdmatrixname-\row-\col.east|-\tikzcdmatrixname-\row-\col.center) to[out=180,in=0] (group\tikzcdmatrixname-\row-\col.west|-\tikzcdmatrixname-\the\numexpr\row+1\relax-\col.center);
	}{
	  \node (group\tikzcdmatrixname-\row-\col) [fit=\LoopGG,operator,inner sep=0pt,label={[gg label,#2]$#4$},#1] {\hphantom{$#4$}};
	}
}

%ghost will get height correct if can't be automatically assigned.
\DeclareExpandableDocumentCommand{\ghost}{O{}O{0pt}O{1.5pt}m}{%optional parameter contains styling info. compulsory is gate text.
	|[inner ysep=4pt,minimum width=#2,minimum height=#3]| \vphantom{#4}
}


%single slice
\newcommand\slice[2][]{%
	%\edef\currcol{\the\pgfmatrixcurrentcolumn}
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
 	\edef\options{\pgfkeysvalueof{/quantikz/style}}
 	\edef\opts{\pgfkeysvalueof{/quantikz/label style}}
	\edef\n{\the\pgfmatrixcurrentcolumn}
	%\expandafter\show\n
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendslices\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\slice@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\n\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}}
%deferred slice command
\newcommand{\slice@end}[4]{
	\edef\top{($1/2*(\tikzcdmatrixname-col#1.east |- \tikzcdmatrixname-row1.north)+1/2*(\tikzcdmatrixname-col\the\numexpr#1+1\relax.west |- \tikzcdmatrixname-row1.north)$)}
	\edef\bottom{($1/2*(\tikzcdmatrixname-col#1.east |- \tikzcdmatrixname-row\the\pgfmatrixcurrentrow.south)+1/2*(\tikzcdmatrixname-col\the\numexpr#1+1\relax.west |- \tikzcdmatrixname-row\the\pgfmatrixcurrentrow.south)+(0,-3pt)$)}
	\expandafter\expandafter\expandafter\make@slice\expandafter\expandafter\expandafter{\expandafter\top\expandafter}\expandafter{\bottom}{#4}{#2}{#3}
}
\newcommand{\make@slice}[5]{
	\draw[slice,#4] #1 to node[pos=0,inner sep=4pt,anchor=south,color=black,#5] {#3} #2;
}
%deferred command which will slice everything
\newcommand{\sliceallr}{
	\edef\sstyle{\pgfkeysvalueof{/tikz/slice style}}
	\edef\slstyle{\pgfkeysvalueof{/tikz/slice label style}}
	\foreach \n in  {2,...,\the\numexpr\pgfmatrixcurrentcolumn-1-\pgfkeysvalueof{/tikz/remove end slices}\relax} {
		\edef\col{\the\numexpr\n-1\relax}
		\edef\title{\pgfkeysvalueof{/tikz/slice titles}}
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\slice@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\n\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\sstyle\expandafter}\expandafter{\slstyle}{\title}
	}
}
%deferred slice command with vertical text
\newcommand{\sliceallvr}{
	\edef\sstyle{\pgfkeysvalueof{/tikz/slice style}}
	\edef\slstyle{\pgfkeysvalueof{/tikz/slice label style}}
	\foreach \n in  {2,...,\the\numexpr\pgfmatrixcurrentcolumn-1-\pgfkeysvalueof{/tikz/remove end slices}\relax} {
		\edef\col{\the\numexpr\n-1\relax}
		\edef\title{\vvv{\pgfkeysvalueof{/tikz/slice titles}}}
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\slice@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\n\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\sstyle\expandafter}\expandafter{\slstyle}{\title}
	}
}

%labelling of inputs
\newcommand\lstick[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
	\pgfkeysgetvalue{/quantikz/label style}{\options}
	\pgfkeysgetvalue{/quantikz/braces}{\opts}
	%\edef\n{\the\pgfmatrixcurrentrow}
	%\edef\m{\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendsavedpaths\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\groupinput@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
%labelling of outputs
\newcommand\rstick[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
	\pgfkeysgetvalue{/quantikz/label style}{\options}
	\pgfkeysgetvalue{/quantikz/braces}{\opts}
	%\edef\n{\the\pgfmatrixcurrentrow}
	%\edef\m{\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendsavedpaths\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\groupoutput@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
%deferred labelling of inputs
\newcommand{\groupinput@end}[4]{%basic data as keys, lable options, brace options, text
	\pgfkeys{/quantikz,wires=1}
 	\pgfkeys{/quantikz,#1}%
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
	\xdef\LoopGI{}
	\foreach \n in  {\row,...,\the\numexpr\row+\quantwires-1\relax} {
	\ifnodedefined{\tikzcdmatrixname-\n-\col}{
		\xdef\LoopGI{\LoopGI(\tikzcdmatrixname-\n-\col)} 
		}{}
		}
	\ifthenelse{\quantwires=1} {
		\node (ingr-\row) [fit=\LoopGI, inner sep=0pt,label={[align=center,#2]left:#4}] {};
	}{
	\node (ingr-\row) [fit=\LoopGI, inner sep=0pt] {};
	\draw[dm,#3] ($(ingr-\row.north west)+(-0.1cm,0.1cm)$) to node[midway,align=center,anchor=east,xshift=-0.1cm,#2] {#4} ($(ingr-\row.south west)+(-0.1cm,-0.1cm)$);
	}
} %
%deferred labelling of outputs
\newcommand{\groupoutput@end}[4]{%basic data as keys, lable options, brace options, text
	\pgfkeys{/quantikz,wires=1}
 	\pgfkeys{/quantikz,#1}%
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
	\xdef\LoopGO{}
	\foreach \n in  {\row,...,\the\numexpr\row+\quantwires-1\relax} {
		\ifnodedefined{\tikzcdmatrixname-\n-\col}{
			\xdef\LoopGO{\LoopGO(\tikzcdmatrixname-\n-\col)} 
		}}
		\ifthenelse{\quantwires=1} {
		\node (outgr-\row) [fit=\LoopGO, inner sep=0pt,label={[align=center,#2]right:#4}] {};
	}{
	\node (outgr-\row) [fit=\LoopGO, inner sep=0pt] {};
	\draw[dd,#3] ($(outgr-\row.north east)+(0.1cm,0.1cm)$) to node[midway,align=center,anchor=west,xshift=0.1cm,#2] {#4} ($(outgr-\row.south east)+(0.1cm,-0.1cm)$);
	}
} %
%inputs and outputs within a multi-wire gate
\newcommand\gateinput[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}%
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
 	\pgfkeysgetvalue{/quantikz/label style}{\options}
 	\pgfkeysgetvalue{/quantikz/braces}{\opts}%
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendlabels\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\mginput@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
\newcommand\gateoutput[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
 	\pgfkeysgetvalue{/quantikz/label style}{\options}
 	\pgfkeysgetvalue{/quantikz/braces}{\opts}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendlabels\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\mgoutput@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
%deferred functions for the above
\newcommand{\mginput@end}[4]{%collected options,label style, brace style,text
	\pgfkeys{/quantikz,wires=1}
 	\pgfkeys{/quantikz,#1}%
 	\edef\quantwires{\pgfkeysvalueof{/quantikz/wires}}
	%\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
%can we find the gategroup node?
\xdef\cell{group\tikzcdmatrixname-1-\col}
\foreach \n in {\row,...,1} {%
	%test if node group-\n-#2 exists
	\ifnodedefined{group\tikzcdmatrixname-\n-\col}{%
    	\xdef\cell{group\tikzcdmatrixname-\n-\col}
    	\breakforeach
	}{}
}
\ifthenelse{\quantwires=1}{%
	\node at ($(\cell.west |- \tikzcdmatrixname-\row-\col.west)+(0,0cm)$)[leftinternal,#2]{#4};
}{%
%\show\quantwires
\draw[dd,#3] ($(\cell.west |- \tikzcdmatrixname-\row-\col.west)+(0.1cm,0.1cm)$) to node[leftinternal,midway,#2] {#4} ($(\cell.west |- \tikzcdmatrixname-\the\numexpr\row+\quantwires-1\relax-\col.west)+(0.1cm,-0.1cm)$);
}
} %
\newcommand{\mgoutput@end}[4]{%
	\pgfkeys{/quantikz,wires=1}
 	\pgfkeys{/quantikz,#1}%
 	\edef\quantwires{\pgfkeysvalueof{/quantikz/wires}}
	%\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
%can we find the gategroup node?
\xdef\cell{group\tikzcdmatrixname-1-\col}
\foreach \n in {\row,...,1} {%
	%test if node group-\n-#2 exists
	\ifnodedefined{group\tikzcdmatrixname-\n-\col}{%
    	\xdef\cell{group\tikzcdmatrixname-\n-\col}
    	\breakforeach
	}{}
}
\ifthenelse{\quantwires=1}{%
	\node at ($(\cell.east |- \tikzcdmatrixname-\row-\col.east)+(0,0cm)$)[rightinternal,#2]{#4};
}{%
\draw[dm,#3] ($(\cell.east |- \tikzcdmatrixname-\row-\col.east)+(-0.1cm,0.1cm)$) to node[rightinternal,midway,#2] {#4} ($(\cell.east |- \tikzcdmatrixname-\the\numexpr\row+\quantwires-1\relax-\col.east)+(-0.1cm,-0.1cm)$);
}
} %

%wave command
\newcommand\wave[1][]{%
	\edef\n{\the\pgfmatrixcurrentrow}
	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendslices\expandafter{%
		\expandafter\wave@end\expandafter{\n}{#1}%
	}
}
%deferred wave
\newcommand{\wave@end}[2]{
	\node (wave-#1) [fit=(\tikzcdmatrixname-row#1),wave,#2] {};
}

%put a border around a group of gates
\newcommand\gategroup[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
 	\pgfkeysgetvalue{/quantikz/style}{\options}
 	\pgfkeysgetvalue{/quantikz/label style}{\opts}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendlabels\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\gategroup@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
%deferred gate group command
\newcommand{\gategroup@end}[4]{%options, gate style, text style, text
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=,steps=1}%
	\edef\background{0}%
	\pgfkeys{/quantikz,#1}%
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}%
	\pgfkeysgetvalue{/quantikz/row}{\row}%
	\pgfkeysgetvalue{/quantikz/col}{\col}%
	\pgfkeysgetvalue{/quantikz/steps}{\steps}%
	\edef\fit{(\tikzcdmatrixname-col\col.west |- \tikzcdmatrixname-row\row.north)(\tikzcdmatrixname-col\the\numexpr\col+\steps-1\relax.east |- \tikzcdmatrixname-row\the\numexpr\row+\quantwires-1\relax.south)}%
	\ifthenelse{\background=1}{%
		\begin{scope}[on background layer]\node (ggroup-\row-\col) [fit=\fit,ggroup,label={[group label,#3]:#4},#2] {};\end{scope}
	}{%
		\node (ggroup-\row-\col) [fit=\fit,ggroup,label={[group label,#3]:#4},#2] {};
	}
}

%use for fudging classical wires that have horizontal and vertical sections
\newcommand{\cwbend}[1]{
	\vcw{#1}\cw
	\edef\cell{\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendlabels\expandafter{%
		\expandafter\latephase@end\expandafter{\cell}
	}
}

\newcommand{\latephase@end}[1]{
	\node [phase,inner sep=2pt] at (\tikzcdmatrixname-#1) {};
}

%patch tikzcd to allow for multiple layers of commands
\patchcmd\tikzcd@{\tikzpicture}{\def\toslice{0}\def\vert{0}
 \begin{tikzpicture}}{}{}
\patchcmd\tikzcd@
    {\global\let\tikzcd@savedpaths\pgfutil@empty}
    {\global\let\tikzcd@savedpaths\pgfutil@empty
    \global\let\tikzcd@atendsavedpaths\pgfutil@empty
    \global\let\tikzcd@atendlabels\pgfutil@empty
    \global\let\tikzcd@atendslices\pgfutil@empty
    \global\let\tikzcd@atendglobals\pgfutil@empty
    \pgfutil@g@addto@macro\tikzcd@savedpaths\DivideRowsCols
    %\pgfmathsetmacro{\mname}{random(100000)}
    \ifthenelse{\toslice=1}{\ifthenelse{\vert=0}{\pgfutil@g@addto@macro\tikzcd@atendslices\sliceallr}{\pgfutil@g@addto@macro\tikzcd@atendslices\sliceallvr}}{}
    }{}{}

%this patching works on modern systems, but I believe is incompatible with the old version that arXiv is running
%\patchcmd\endtikzcd{\tikzcd@savedpaths}{\tikzcd@savedpaths\tikzcd@atendsavedpaths\tikzcd@atendlabels\tikzcd@atendslices{\globaldefs=1\tikzcd@atendglobals}}{}{}

%instead, completely redefine the function
\def\endtikzcd{%
  \pgfmatrixendrow\egroup%
  \pgfextra{\global\let\tikzcdmatrixname\tikzlastnode};%
  \tikzcdset{\the\pgfmatrixcurrentrow-row diagram/.try}%
  \begingroup%
    \pgfkeys{% `quotes' library support
      /handlers/first char syntax/the character "/.initial=\tikzcd@forward@quotes,%
      /tikz/edge quotes mean={%
        edge node={node [execute at begin node=\iftikzcd@mathmode$\fi,%$
                         execute at end node=\iftikzcd@mathmode$\fi,%$
                         /tikz/commutative diagrams/.cd,every label,##2]{##1}}}}%
    \let\tikzcd@errmessage\errmessage% improve error messages
    \def\errmessage##1{\tikzcd@errmessage{##1^^J...^^Jl.\tikzcd@lineno\space%
        I think the culprit is a tikzcd arrow in cell \tikzcd@currentrow-\tikzcd@currentcolumn}}%
    \tikzcd@before@paths@hook%
    \tikzcd@savedpaths\tikzcd@atendsavedpaths\tikzcd@atendlabels\tikzcd@atendslices{\globaldefs=1\tikzcd@atendglobals}%I just added stuff here instead
  \endgroup%
  \end{tikzpicture}%
  \ifnum0=`{}\fi}


%end patching
%\makeatother

%this command runs after we've finished the matrix, and makes unified cells for each row and each column. This allows much nicer alignment of large boxes.
\newcommand{\DivideRowsCols}{
	\foreach \n in {1,...,\the\pgfmatrixcurrentrow} {%for each row, construct a master cell that contains all entries
	\xdef\LoopRow{}
		\foreach \m in {1,...,\the\pgfmatrixcurrentcolumn}{
			\ifnodedefined{\tikzcdmatrixname-\n-\m}{
				\xdef\LoopRow{\LoopRow(\tikzcdmatrixname-\n-\m)}
			}{}
			\ifnodedefined{group\tikzcdmatrixname-\n-\m}{
				\xdef\LoopRow{\LoopRow(group\tikzcdmatrixname-\n-\m)}
			}{}
	}
	\node (\tikzcdmatrixname-row\n) [fit=\LoopRow] {};
	}
	\foreach \n in {1,...,\the\pgfmatrixcurrentcolumn} {%for each column, construct a master cell that contains all entries
	\xdef\LoopCol{}
		\foreach \m in {1,...,\the\pgfmatrixcurrentrow}{
			\ifnodedefined{\tikzcdmatrixname-\m-\n}{
				\xdef\LoopCol{\LoopCol(\tikzcdmatrixname-\m-\n)}
			}{}
			\ifnodedefined{group\tikzcdmatrixname-\m-\n}{
				\xdef\LoopCol{\LoopCol(group\tikzcdmatrixname-\m-\n)}
			}{}
	}
	\node (\tikzcdmatrixname-col\n) [fit=\LoopCol] {};
	}
}

%initialise all the pgfkeys for key=value parametre passing in macro options

\pgfkeys{/tikz/slice all/.code={\def\toslice{1}},/tikz/remove end slices/.initial=0,/tikz/slice titles/.initial={\col},/tikz/slice style/.initial={},/tikz/slice label style/.initial={},/tikz/thin lines/.code={\resetstyles},/tikz/transparent/.code={\maketransparent},/tikz/vertical slice labels/.code={\def\vert{1}}}
\pgfkeys{/quantikz/.is family,/quantikz,%
.unknown/.style={%
	/quantikz/wires=\pgfkeyscurrentname
},%
wires/.initial=1,%
style/.initial={},label style/.initial={},braces/.initial={},background/.code={\def\background{1}},alternate/.code={\def\helper{1}},row/.initial=1,col/.initial=1,steps/.initial=1,Strike Width/.initial=0.08cm,Strike Height/.initial=0.12cm,swap/.code={\def\toswap{1}},disable auto height/.code={\def\DisableMinSize{1}},cwires/.initial={-1},nwires/.initial={-1}}

%my standard Dirac notation commands. can be overridden by user.
\providecommand{\ket}[1]{\ensuremath{\left|#1\right\rangle}}
\providecommand{\bra}[1]{\ensuremath{\left\langle#1\right |}}
\providecommand{\proj}[1]{\ensuremath{\ket{#1}\!\bra{#1}}}
\providecommand{\braket}[2]{\ensuremath{\left\langle#1\middle|#2\right\rangle}}

%single qubit operations
\newcommand{\phantomgate}[1]{|[linecont,thickness, inner ysep=3pt]| \phantom{#1} \qw}
\newcommand{\hphantomgate}[1]{|[linecont,minimum size=1.5em,thickness]| \hphantom{#1} \qw}
%\newcommand{\push}[1]{#1 \qw}
\newcommand{\alias}[1]{|[alias=#1]|}
\DeclareExpandableDocumentCommand{\phase}{O{}m}{|[phase,#1,label={[phase label,#1]#2}]| {} \qw}
\DeclareExpandableDocumentCommand{\control}{O{}m}{|[phase,#1]| {} \qw}
\DeclareExpandableDocumentCommand{\ocontrol}{O{}m}{|[ophase,#1]| {} \qw}
\DeclareExpandableDocumentCommand{\targ}{O{}m}{|[circlewc,#1]| {} \qw}
\DeclareExpandableDocumentCommand{\targX}{O{}m}{|[crossx2,#1]| {} \qw}
\newcommand{\linethrough}{|[linecont, inner ysep=3pt]| }

%measuring
\DeclareExpandableDocumentCommand{\meter}{O{}{m}}{|[meter,label={[my label]#2},#1]| {} \qw}
\DeclareExpandableDocumentCommand{\measuretab}{O{}{m}}{|[measuretab,#1]| {#2} \qw}
\DeclareExpandableDocumentCommand{\meterD}{O{}{m}}{|[meterD,#1]| {#2} \qw}
\DeclareExpandableDocumentCommand{\measure}{O{}{m}}{|[measure,#1]| {#2} \qw}

%controlled gates
\def\ctrl#1{\control{}	\vqw{#1}}
\def\octrl#1{\ocontrol{}\vqw{#1}}
\def\swap#1{%
	\targX{}
	\edef\start{\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
	\edef\end{\the\numexpr#1+\pgfmatrixcurrentrow\relax-\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\vqwexplicitcenter\expandafter\expandafter\expandafter{\expandafter\start\expandafter}\expandafter{\end}
}

%vertical wires
%classical vertical wire, relative positioning
\newcommand{\vcw}[1]{
	\edef\start{\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
	\edef\end{\the\numexpr#1+\pgfmatrixcurrentrow\relax-\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\vcwexplicit\expandafter\expandafter\expandafter{\expandafter\start\expandafter}\expandafter{\end}
}
%vertical quantum wire, relative positioning
\newcommand{\vqw}[1]{
	\edef\start{\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
	\edef\end{\the\numexpr#1+\pgfmatrixcurrentrow\relax-\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\vqwexplicit\expandafter\expandafter\expandafter{\expandafter\start\expandafter}\expandafter{\end}
}
%quantum wire, absolute positioning
\newcommand{\vqwexplicit}[2]{
	\arrow[from=#1,to=#2,arrows] {}
}
%classical vertical wire, absolute positioning
\newcommand{\vcwexplicit}[2]{
	\arrow[from=#1,to=#2,arrows,xshift=0.05cm] {}\arrow[from=#1,to=#2,arrows,xshift=-0.05cm] {}
}
%classical horizontal wire, absolute positioning
\newcommand{\vcwhexplicit}[2]{
	\arrow[from=#1,to=#2,arrows,yshift=0.05cm] {}\arrow[from=#1,to=#2,arrows,yshift=-0.05cm] {}
}
%quantum wire, absolute positioning, going to centres of cell, not edge.
\newcommand{\vqwexplicitcenter}[2]{
	\arrow[from=#1,to=#2,arrows,start anchor=center,end anchor=center] {}
}

%horizontal wires
\newcommand{\qw}{\ifthenelse{\the\pgfmatrixcurrentcolumn>1}{\arrow[arrows]{l}}{}}
\newcommand{\cw}{\ifthenelse{\the\pgfmatrixcurrentcolumn>1}{\arrow[arrows,yshift=0.05cm]{l}\arrow[arrows,yshift=-0.05cm]{l}}{}}
%define the strike distance for strike-through on qwbundle.
%\newcommand*{\StrikeDistance}{0.1cm}%
%a bundle of horizontal quantum wires
\newcommand{\qwbundle}[2][]{\ifthenelse{\the\pgfmatrixcurrentcolumn>1}{
	\def\helper{0}
	\pgfset{/quantikz,#1}
	\ifthenelse{\helper=1}{
		\arrow[arrows,yshift=0.1cm]{l}\arrow[arrows]{l}\arrow[arrows,yshift=-0.1cm]{l}
	}{
	\arrow[phantom,strike arrow]{l}[xshift=\pgfkeysvalueof{/quantikz/Strike Width}, yshift=\pgfkeysvalueof{/quantikz/Strike Height},anchor=south west,inner sep=0pt]{\scriptstyle #2}
	}}{}}




%configure some of the style properties.
\tikzcdset{row sep/normal=0.5cm,column sep/normal=0.5cm,thick,nodes in empty cells,
	every cell/.style={
        anchor=center,minimum size=0pt,inner sep=0pt,outer sep=0pt,thick
    },
    arrows/.style={dash,thick},
    1-row diagram/.style={}
    }
\tikzset{
	thickness/.style={thick},
    operator/.style={draw,fill=white,minimum size=1.5em, inner sep=2pt,thickness,align=center},
    ggroup/.style={draw,minimum size=1.5em,thickness,align=center,inner sep=4pt},
    leftinternal/.style={anchor=mid west,font=\scriptsize,inner sep=4pt,align=center},
    rightinternal/.style={anchor=mid east,font=\scriptsize,inner sep=4pt,align=center},
    wave/.style={inner sep=-3pt,tape,fill=white,apply={draw=black} except on segments {5,6,1,2,9}},
    phase/.style={fill,shape=circle,minimum size=4pt},
    phase label/.style={label distance=2mm,anchor=mid,label position=45},
    ophase/.style={fill=white,draw=black,shape=circle,minimum size=4pt},
    internal/.style={thickness,black},
    line/.style={path picture={ 
\draw[internal](path picture bounding box.west) -- (path picture bounding box.east);
}},
	linecont/.style={circle,line},
    cross/.style={path picture={ 
\draw[internal](path picture bounding box.north) -- (path picture bounding box.south) (path picture bounding box.west) -- (path picture bounding box.east);
}},
    circlewc/.style={draw,circle,cross,minimum width=4pt,inner sep=3pt},
    crossx/.style={path picture={ 
\draw[internal,inner sep=0pt]
(path picture bounding box.south east) -- (path picture bounding box.north west) (path picture bounding box.south west) -- (path picture bounding box.north east) (path picture bounding box.west) -- (path picture bounding box.east);
}},
	crossx2/.style={circle,crossx,minimum size=1em},
    dd/.style={decoration={brace},decorate,thickness},
    dm/.style={decoration={brace,mirror},decorate,thickness},
    slice/.style={thickness,red,dash pattern=on 5pt off 3pt,align=center},
    meter/.style={draw,fill=white,minimum width=2em,minimum height=1.5em, rectangle, font=\vphantom{A}, thickness,
 path picture={\draw[black] ([shift={(.1,.24)}]path picture bounding box.south west) to[bend left=50] ([shift={(-.1,.24)}]path picture bounding box.south east);\draw[black,-{Latex[scale=0.6]}] ([shift={(0,.1)}]path picture bounding box.south) -- ([shift={(.3,-.1)}]path picture bounding box.north);}},
 	measuretab/.style={draw,signal,signal to=west,inner sep=4pt,fill=white},
 	meterD/.style={draw,rounded rectangle,rounded rectangle left arc=none,inner sep=4pt,fill=white},
 	measure/.style={draw,rounded rectangle,inner sep=4pt,fill=white},
 	my label/.style={yshift=0.1cm,above,align=center},
 	gg label/.style={label position=center,align=center},
 	group label/.style={label position=above,yshift=0.2cm,anchor=mid},
 	strike arrow/.style={
    decoration={markings, mark=at position 0.5 with {
        \draw [internal,-] 
            ++ (-\pgfkeysvalueof{/quantikz/Strike Width},-\pgfkeysvalueof{/quantikz/Strike Height} )
            -- ( \pgfkeysvalueof{/quantikz/Strike Width}, \pgfkeysvalueof{/quantikz/Strike Height});}	%can I use pgfkeys and do some maths here?
    },
    postaction={decorate},
}
}

\def\resetstyles{
\tikzcdset{thin,every cell/.append style={thin},arrows/.append style={thin}
    }
\tikzset{
	thickness/.style={thin},
	%operator/.append style={thin},
	%internal/.append style={thin},
	%dd/.append style={thin},
	%dm/.append style={thin},
	%slice/.append style={thin},
	meter/.append style={thin},
	phase/.append style={minimum size=3pt},
	ophase/.append style={minimum size=3pt},
	%circlewc/.append style={minimum size=3pt,inner sep=2pt}
}
}

\def\maketransparent{
\tikzset{
	operator/.append style={fill opacity=0},
	meter/.append style={fill opacity=0}
}
}
